Observation of a level crossing in a molecular nanomagnet using implanted muons

We have observed an electronic energy level crossing in a molecular nanomagnet (MNM) using muon-spin relaxation. This effect, not observed previously despite several muon studies of MNM systems, provides further evidence that the spin relaxation of the implanted muon is sensistive to the dynamics of the electronic spin. Our measurements on a broken ring MNM [H_{2}N^{t}Bu^{is}Pr][Cr_{8}CdF_{9}(O_{2}CC(CH_{3})_{3})_{18}] (hereafter Cr_{8}Cd), which contains eight Cr ions, show clear evidence for the S=0 to S=1 transition that takes place at B_{c}=2.3 T. The crossing is observed as a resonance-like dip in the average positron asymmetry and also in the muon-spin relaxation rate, which shows a sharp increase in magnitude at the transition and a peak centred within the S=1 regime.

==> PaxHeader/mlc.tex <==
17 gid=784332012
17 uid=565286453
20 ctime=1303307627
20 atime=1303307635
38 LIBARCHIVE.creationtime=1303112633
24 SCHILY.dev=234881026
21 SCHILY.ino=179843
18 SCHILY.nlink=1

